M3A: Model, MetaModel, and Anomaly Detection in Web Searches

'Alice' is submitting one web search per five minutes, for three hours in a row - is it normal? How to detect abnormal search behaviors, among Alice and other users? Is there any distinct pattern in Alice's (or other users') search behavior? We studied what is probably the largest, publicly available, query log that contains more than 30 million queries from 0.6 million users. In this paper, we present a novel, user-and group-level framework, M3A: Model, MetaModel and Anomaly detection. For each user, we discover and explain a surprising, bi-modal pattern of the inter-arrival time (IAT) of landed queries (queries with user click-through). Specifically, the model Camel-Log is proposed to describe such an IAT distribution; we then notice the correlations among its parameters at the group level. Thus, we further propose the metamodel Meta-Click, to capture and explain the two-dimensional, heavy-tail distribution of the parameters. Combining Camel-Log and Meta-Click, the proposed M3A has the following strong points: (1) the accurate modeling of marginal IAT distribution, (2) quantitative interpretations, and (3) anomaly detection.

==> discussion.tex <==
\begin{observation}[In-session and take-off]
The median in-session IAT is about five minutes, whereas the median of take-off IAT is approximately seven hours.
\end{observation}
We begin the discussion with the interpretation of in-session and take-off behaviors. The median IAT of in-session queries is about 5 minutes, which approximately represents the duration a user interested in the query results. On the other hand, the IAT of take-off queries is longer, ranging from tens of minutes (\eg, lunch break), hours (\eg, sleep time), to days (\eg, weekends). The median IAT of take-off queries is approximately seven hours, which corresponds to sleep time very well.

\begin{observation}[Common user behavior]
The mode of the ratio $\Ratio$ is approximately three, which suggests a common user behavior: ``click, click, click, and then go away.''
\end{observation}

Thanks to \mll's generativity and interpretability, the marginal distribution of IAT from a user is now characterized by five parameters. Therefore, we can answer `what-if' scenario by changing the values of each parameter. Also, we would like to mention the mode of the ratio $\Ratio$ is approximately three, as observed in Fig.~\ref{fig:Validation of marginal distribution of parameter}(a), which suggests a common user behavior: ``query-click, query-click, go away.''

Also thanks to \cop's detectability, less obvious anomalies can now be spotted. Since \cop models the joint distribution of $\Ratio$ and $\Mean$, it can be used to calculate the likelihood of observing an anomaly (outlier).


==> makefile <==
paper.pdf: paper.tex
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper

clean:
	\rm -f *.aux *.log *.dvi *.bbl *.blg

spotless: clean
	\rm -f paper.pdf

